Language Models with Rationality

While large language models (LLMs) are proficient at question-answering (QA), it is not always clear how (or even if) an answer follows from their latent "beliefs". This lack of interpretability is a growing impediment to widespread use of LLMs. To address this, our goals are to make model beliefs and their inferential relationships explicit, and to resolve inconsistencies that may exist, so that answers are supported by interpretable chains of reasoning drawn from a consistent network of beliefs. Our approach, which we call REFLEX, is to add a rational, self-reflecting layer on top of the LLM. First, given a question, we construct a belief graph using a backward-chaining process to materialize relevant model beliefs (including beliefs about answer candidates) and their inferential relationships. Second, we identify and minimize contradictions in that graph using a formal constraint reasoner. We find that REFLEX significantly improves consistency (by 8%-11% absolute) without harming overall answer accuracy, resulting in answers supported by faithful chains of reasoning drawn from a more consistent belief system. This suggests a new style of system architecture in which an LLM extended with a rational layer can provide an interpretable window into system beliefs, add a systematic reasoning capability, and repair latent inconsistencies present in the LLM.

==> results-tables.tex <==


\begin{table}[t]
\centering
{\small
\setlength{\tabcolsep}{2pt}	%
\begin{tabular}{l|c|c|c} \hline
   & Entail- &  &  \\
System & mentBank & OBQA & Quartz \\ \hline  
LLM & 87.0 & 88.2 & 85.7\\ 
LLM + rational layer (\sysname) & \textbf{96.1} & \textbf{95.9} & \textbf{96.6} \\
\hline
\end{tabular}
}
\hspace{1ex} \\
\hspace{1ex} \\ %
{
\setlength{\tabcolsep}{2pt}	%
\begin{tabular}{l|c|c|c} \hline
   & Entail- &  &  \\
System & mentBank & OBQA & Quartz \\ \hline  
LLM & 87.0 & 88.2 & 85.7\\ 
LLM + rational layer & \multirow{2}{*}{\textbf{96.1}} & \multirow{2}{*}{\textbf{95.9}} & \multirow{2}{*}{\textbf{96.6}} \\
\multicolumn{1}{l|}{\ \ \ (\sysname)} & & \\
\hline
\end{tabular}
}
    \caption{{\bf Consistency:} By adding a rational layer to our baseline LLM, \sysname significantly improves
      consistency among beliefs by resolving uncovered conflicts.}  %
\label{Results-overall}
\end{table}

\begin{table}[t]
\centering
    {\small
\setlength{\tabcolsep}{2pt}	%
\begin{tabular}{l|c|c|c} \hline
   & Entail- &  &  \\
System & mentBank & OBQA & Quartz \\ \hline  
LLM & 79.4 & 74.0 & 80.2\\ 
LLM + rational layer (\sysname) & 79.9 & 75.0 & 80.0 \\ 
\hline
\end{tabular}
}
\caption{{\bf QA accuracy:} \sysname's belief revision in the rational layer preserves overall QA accuracy.}
\label{Results-acc}
\end{table}

\begin{table}[t]
\centering
    { %
\begin{tabular}{lc} \hline
  System & EntailmentBank \\ \hline
\sysname (our system): & 96.1 \\
\hspace*{3mm} - without $p \rightarrow h$ rules & 93.8 \\
\hspace*{3mm} - without XOR rules & 90.4 \\
\hspace*{3mm} - without MC rule & 95.8 \\
\hline
\end{tabular}
}
    \caption{{\bf Consistency:} Ablations on EntailmentBank (Dev) suggest that all three types of rule contribute to improving self-consistency.
  \label{Results-ablation-type}}
\end{table}


